Linear-Depth Quantum Circuits for n-qubit Toffoli gates with no Ancilla

We design a circuit structure with linear depth to implement an $n$-qubit Toffoli gate. The proposed construction uses a quadratic-size circuit consists of elementary 2-qubit controlled-rotation gates around the x axis and uses no ancilla qubit. Circuit depth remains linear in quantum technologies with finite-distance interactions between qubits. The suggested construction is related to the long-standing construction by Barenco et al. (Phys. Rev. A, 52: 3457-3467, 1995, arXiv:quant-ph/9503016), which uses a quadratic-size, quadratic-depth quantum circuit for an $n$-qubit Toffoli gate.

==> figures/T4.tex <==
$$
\Qcircuit @C=1em @R=0.5em @!R{
\lstick{a_1}	&\qw			&\qw				&\ctrl{1}				&\qw				&\qw			&\qw			&\ctrl{1}			&\qw			&\qw	&\rstick{a_1}		\\
\lstick{a_2}   	&\qw			&\ctrl{1}				&\gate{\pi}\qwx			&\ctrl{1}				&\qw			&\ctrl{1}			&\gate{-\pi}\qwx		&\ctrl{1}			&\qw	&\rstick{a_2}   		\\
\lstick{a_3}   	&\ctrl{1}			&\gate{\frac{\pi}{2}}\qwx		&\gate{\frac{\pi}{2}}\qwx		&\gate{\frac{-\pi}{2}}\qwx		&\ctrl{1}			&\gate{\frac{\pi}{2}}\qwx	&\gate{\frac{-\pi}{2}}\qwx	&\gate{\frac{-\pi}{2}}\qwx	&\qw	&\rstick{a_3} 		\\
\lstick{a_4}   	&\gate{\frac{\pi}{2}}\qwx	&\gate{\frac{\pi}{4}}\qwx		&\gate{\frac{\pi}{4}}\qwx		&\gate{\frac{-\pi}{4}}\qwx		&\gate{\frac{-\pi}{2}}\qwx	&\qw			&\qw			&\qw			&\qw	&\rstick{a_1a_2a_3 \oplus a_4}	\gategroup{4}{7}{4}{9}{1em}{_\}}	\\
}															 																				
$$
